Localization in 1D non-parametric latent space models from pairwise affinities

We consider the problem of estimating latent positions in a one-dimensional torus from pairwise affinities. The observed affinity between a pair of items is modeled as a noisy observation of a function $f(x^*_{i},x^*_{j})$ of the latent positions $x^*_{i},x^*_{j}$ of the two items on the torus. The affinity function $f$ is unknown, and it is only assumed to fulfill some shape constraints ensuring that $f(x,y)$ is large when the distance between $x$ and $y$ is small, and vice-versa. This non-parametric modeling offers a good flexibility to fit data. We introduce an estimation procedure that provably localizes all the latent positions with a maximum error of the order of $\sqrt{\log(n)/n}$, with high-probability. This rate is proven to be minimax optimal. A computationally efficient variant of the procedure is also analyzed under some more restrictive assumptions. Our general results can be instantiated to the problem of statistical seriation, leading to new bounds for the maximum error in the ordering.

==> modifs.tex <==
%%%%%%%%%
%% changements
%%%%%%%%%

%\subsection*{Reste \`a reprendre dans seriation-main}
%\begin{itemize}
%\item \sout{abstract \ch{j'ai retir\'e toute r\'ef\'erence \`a embedding car \c{c}a me semblait glissant} + titre \ch{on a envie de mettre point localization / pairwise affinities / 1D / non-parametric / latent space model. Ca fait un peu trop? proposition \`a discuter} \ya{Montanari a mis 'Localization' sans 'point' :) Suggestion de titre: 'Localization in 1D-space: a nonparametric point of view', ou 'Localization in 1D latent space from a nonparametric viewpoint', ou 'A nonparametric approach to unidimensional localization', ou 'A nonparametric view of Localization  in 1D latent space model'}}
%\item \sout{related work + biblio matching d\'ebut intro}
%\item \sout{discussion related work seriation}
%\item \sout{problemes de notations (remarques de Yann)}
%\item \sout{optim procruste} \ch{pas trouv\'e de r\'ef\'erence  \`a ce probl\`eme pr\'ecis (norme), j'ai donc pr\'ef\'er\'e retirer cette mention}
%\item section num\'erique
%\item \sout{Insister dans la section 3.2 que $\hat{x}^{(1)}_S$ est dans $\bPi_{n_0}$.}
%\item Probabilite en $1/n$ plutot que $1/n_0$ dans les enonce? [Verifier les proba dans toute les combinaisons de proba spectral (Theorem 4 et co ... ) ]
%\end{itemize}


%\subsection*{Changement de notations et terminologie}
%\begin{itemize}
%\item \sout{Question sur les notations: difference en constantes $c$ and $C$}
%\item \sout{space $X$ devient $\mathcal{X}$} \nv{ok}
%\item \sout{$\tilde f$ devient $g$ pour les graphes g\'eom\'etrique} \ya{fait}
%\item \sout{il y avait un autre $\tilde f$ dans la proposition \ref{prop_identif}. Je l'ai chang\'e en $f'$. J'ai aussi chang\'e $\tilde \xbf$ en $\xbf'$.} \nv{ok}
%\item \sout{$\alpha({\bf x})$ devient $d({\bf x},\Pi_{n})$} \ya{ $\alpha$ est introduit ds l'append spectral}\nv{nico:je les ai remplace partout}
%\item \sout{l'equation de label {example:identif} qui disait $\tilde{f}(\tilde{x}_i,\tilde{x}_j) = f(x_i,x_j)\, , \text{ for all }i,j\in[ n]$ dans la proposition \ref{prop_identif} a disparue.} \nv{ok}
%\item \sout{dans la section 3.2 l'estimation pr\'eliminaire est not\'ee $\xbf^{(1)}_{S}$ au lieu de $\xbf_{S}$. Une petite phrase pr\'eliminaire dans la preuve devrait faire l'affaire.  \nv{normalement c'est bon}}
%\item \sout{Le proposition de label {prop:LHO:perf:motiv} a disparu (trop redondante) }
%\item \sout{le preliminary estimator (section \ref{estimL1}, Proposition \ref{l1bound}) est maintenant not\'e $\hxbf_{S}^{(1)}$.} \nv{ok}
%\item \sout{les notations $\hat x^{(1)}$ et $\hat x^{(2)}$ \'etaient utilis\'es pour la r\'ep\'etition du sampling. Pour eviter une confusion entre \'etape 1 = localisation, \'etape 2 = refinement, et les 2 \'etapes de sampling, j'ai remplac\'e partout $S_{1}, S_{2}$ etc, par $S,S'$ etc. A priori, le changement est assez localis\'e. } \nv{ok}
%\item \sout{Attention \`a $D(\xbf)$ chang\'e en  $D(\xbf_{S})$ car sinon probl\`eme d'indices} \nv{ok}
%\item \sout{pour le vanilla spectral, j'ai chang\'e $\hxbf'$ en $\hxsp$} \ya{ok}
%\item pour all\'eger $z_{i}$ remplace $x_i^{(p)}$ dans Uniform Approximation. J'ai aussi chang\'e la formulation de l'algo, il faudra accorder la preuve \ya{fait (UA est repris en toute généralité ds append spec)}
%\item Corollaire \ref{cor:spectral} est fusionn\'e avec Prop \ref{conj:graphgeo:l1} \ya{ok}
%\item \ya{notations ds l'append spectral, qui diffèrent de celles du Main : $F_{(\textbf{x}^*,f)}$ au lieu de $F$, idem $F_{(\textbf{x}^*_S,f)}$ au lieu de $F_{SS}$ (cette notation a été supprimé de lapend spectral, sauf ds un petit lemme technique tt à la fin, c'est OK comme ça pour moi);} %J'ai gardé le symbole $\lesssim_{c_l,c_L,c_e,c_a}$ mais ne sais pas s'il est défini qlq part; 
%Espace produit $\mathcal{C}^{\times n}$ au lieu de $\mathcal{C}^n$ (la notation $\mathcal{C}^{\times n}$ a été supprimé ds l'append spectral)
%\item \ya{attention aux notations mentionnées au point précédent, elles apparaissent peut être dans d'autres appendices que le spectral}
%\item \ya{norme 1 et 2 sont utilisées dans Uniform Approximation. Quest: introduit-on ces norme juste avant l'algo UA ? (rmq: norme 1 et 2 sont déjà introduites dans la ss-section notation)}
%\end{itemize}





%\subsection*{preuves \`a mettre \`a jour}
%\begin{itemize}
%\item \sout{reprendre preuve Lemma~\ref{lem:regret} en s'appuyant sur Lemma~\ref{lem:conerstone:variante} ? d'autres endroits aurait pu s'y pr\^eter (pour le refinement) mais les preuves actuelles sont \'ecrites assez diff\'eremment.}
%\item on a $\xbf\in\Ccal^n$, mettre un petit mot partout o\`u $\xbf$ vu comme une matrice $2\times n$ (typiquement les bornes en distance $d_{1}$). \nv{Il reste a mettre des petits mots pour la partie spectrale. }
%\item Le preuve de la Proposition \ref{prop:representative} est \`a r\'ediger. La partie $c_{e}=0$, $\xbf,\xbf'\in\bPi_{n}$ pourrait rejoindre l'appendix \ref{app:central}, car c'est un point clef (et \c{c}a se prouve \`a l'aide de Lemma~\ref{lem:conerstone:variante}). 
%\sout{Le cas g\'en\'eral est quant \`a lui une cons\'equence du Theorem \ref{lem:collage}}
%\item  \sout{dans le th\'eor\`eme \ref{thm:principal} j'ai du passer de $\xbf^*$ \`a $\xbf$, voir si impact dans les preuves.} 
%\item voir terme diagonal dans preuve spectral (partie signal) \ya{fait}
%\item inclure une preuve pour noiseless case section 3.2 ?
%\item \sout{cet \'enonc\'e \`a disparu dans la nouvelle version au profit du Theorem \ref{thm:principal}, mais peut \^etre veut-on le conserver dans les preuves?}
%\item j'ai retir\'e ce lemme de la section 4, \`a mettre en appendice \ya{ok}
%\begin{lem}\label{lem:approx:estimPos}For any ${\bf x}_S\in \mathbb{R}^{ 2 \times n_0}$ and any ${\bf x}^*_{S}\in \Ccal^{\times n_0}$, the vector $\widetilde{{\bf x}}_S\in \bPi_{n_0}$ returned by UA satisfies
%\begin{equation*}
%    \|\widetilde{{\bf x}}_S - {\bf x}^*_{S}\|_{1,\Ocal} \lesssim  \|{\bf x}_S - {\bf x}^*_{S}\|_{1,\Ocal} + n \alpha({\bf x}^*_{S}) + 1\enspace .
%\end{equation*}
%\end{lem}
%\item pour les r\'esultats avec le spectral, il faut v\'erifier que les gaps spectraux de $F$ et $F_{S}$ ont bien \'et\'e reli\'es pour $S$ tir\'e uniform\'em\'ent. \ya{fait}
%\item la proposition \ref{thm:graphgeo} concerne maintenant l'estimation compl\`ete et pas seulement ce qui se passe sur $S$. Petit update \`a pr\'evoir car la condition \eref{GraphGeo:assump:latentPosition} porte d\'esormais sur $\xbf^*$ et non $\xbf^*_{S}$. Pour le reste, juste 3 phrases \`a ajouter a priori. \ya{ok}
%\end{itemize}


%\subsection*{Divers \`a faire}
%\begin{itemize}
%\item \sout{A voir: titre section 1.1. / 1D latent space model.}
%\end{itemize}
